The Ubiquitous Skiplist: A Survey of What Cannot be Skipped About the Skiplist and its Applications in Big Data Systems

Skiplists have become prevalent in systems. The main advantages of skiplists are their simplicity and ease of implementation, and the ability to support operations in the same asymptotic complexities as their tree-based counterparts. In this survey, we explore skiplists and their many variants. We highlight many scenarios about how skiplists are useful, and how they fit well in these usage scenarios. We also compare skiplists with other data structures, especially tree-based structures. Extensions to skiplists include structural modifications, as well as algorithmic enhancements and operations. We categorize the existing extensions, and summarize the skiplist variants that belong to each category. We present how data systems incorporate skiplist variants into many different application scenarios to serve various purposes. These data systems cover a wide range of applications, from data indexing to block-chain, from network algorithms to deterministic skiplists, etc. It illustrates an impactful and diverse applications of skiplists in various domains of data systems.

==> figs/chart.tex <==
\newcommand\yx{0}
\newcommand\ya{1}
\newcommand\yb{3}
\newcommand\yc{4.5}
\newcommand\yd{6}
\newcommand\ye{7.5}
\newcommand\yf{9}
\newcommand\yg{10.5}
\newcommand\yh{12}

\newcommand\topy{10}

% \setlist{year}{'17a, '18b, '19c, '20d, '21e, '22f, '23g, '24h}
% \setlist{xpos}{\ya, \yb, \yc, \yd, \ye, \yf, \yg, \yh}
% Create position for each year from the xpos list and create commands
\newcommand\NS{2mm}
\newcommand\NC{1mm}
\usetikzlibrary {automata, positioning}
\usetikzlibrary{shapes.geometric} % For ellipse, diamond, trapezium, etc.

% \resizebox{\linewidth}{!}{
\begin{tikzpicture}[
    shorten >=1pt,
    node distance=2cm,
    on grid,
    auto,
    % unique nodes
    spatial/.style={circle, draw=black, fill=black!50, very thick, minimum size=\NC},
    st-past/.style={circle, draw=black, very thick, minimum size=\NC},
    st-curr/.style={circle, draw=black, fill=black!5, very thick, minimum size=\NC},
    st-fut/.style={circle, draw=black, fill=black!25, very thick, minimum size=\NC},
    s-txt/.style={rectangle, draw=black, very thick, minimum size=\NS},
    st-txt/.style={rectangle, draw=black, fill=black!25, very thick, minimum size=\NS},
    unknown/.style={rectangle, draw=red, fill=red!25, very thick, minimum size=\NS},
    % skiplist
    default/.style={circle, draw=black, fill=black!50, very thick, minimum size=\NC},
    deter/.style={rectangle, draw=black, very thick, minimum size=\NC},
    concur/.style={circle, draw=black, very thick, minimum size=1.2mm},
    other/.style={trapezium, draw=black, very thick, minimum size=\NC},
    index/.style={trapezium, draw=black, fill=black!50, very thick, minimum size=\NC},
    % paths
    paths/.style={->, ultra thick, >=stealth'},
    every node/.style={font=\scriptsize}]
]

% ================================================================================================
% help line
\draw[help lines,xstep=0.25cm,ystep=0.25cm] (0,0) grid (17, 10);
% ================================================================================================
% draw nodes 

% ==============================
% parents
\node[spatial,label={[align=center]below:Spatial\\Pyramid\\\cite{10.1145/1007568.1007637}}]      (spy)     at(\yx,1)    {};
\node[s-txt,label={[align=center]below:CIR-Tree\\\cite{10.14778/1687627.1687666}}]      (cir)     at(\yx,2)    {};
\node[unknown,label={[align=center]below:vEB-Tree\\\cite{cormen2009introduction}}]      (veb)     at(\yx,3)    {};
\node[spatial,label={[align=center]below:R-Tree\\\cite{10.1145/971697.602266}}]      (r)     at(\yx,4)    {};
\node[spatial,label={[align=center]below:Spatial\\Grid~\cite{10.1145/348.318586}}]      (sgrid)     at(\yx,5)    {};

\node[default,label={[align=center]below:SkipList\\\cite{pugh1990skip}}]      (skiplist)     at(\yx,\topy)    {};
\node[default,label={[align=center]below:Interval\\\cite{hanson1991interval}}]      (interval)     at(\yx+0.5, \topy-0.5)    {};
\node[deter,label={[align=center]below:Deterministic\\\cite{munro1992deterministic}}]      (deter)     at(\yx+1, \topy-1)    {};

% ==============================
% 1996
\node[default,label={[align=center]below:B+-tree\\Comparison\\\cite{lamoureux1996equivalence}}]      (btreecmp)     at(\yx+3, \topy-1)    {};

% ==============================
% 1998
\node[default,label={[align=center]below:Multi-dim\\\cite{nickerson1998skip}}]      (multidim)     at(\yx+4, \topy-1)    {};
\node[concur,label={[align=center]below:Lock-based\\\cite{pugh1998concurrent}}]      (concur)     at(\yx+4, \topy-2)    {};

% ==============================
% 2001
\node[default,label={[align=center]below:Biased\\Skiplist\\\cite{ergun2001biased}}]      (biased)     at(\yx+5.5, \topy-1)    {};

% ==============================
% 2003
\node[concur,label={[align=center]below:Practical\\Lock-freedom}]      (freedom)     at(\yx+6.5, \topy-1)    {};
\node[concur,label={[align=center]below:Lock-free\\\cite{sundell2005fast}}]      (lockfree)     at(\yx+6.5, \topy-2)    {};
\node[other,label={[align=center]below:SkipNet\\\cite{harvey2002skipnet}}]      (skipnet)     at(\yx+6.5, \topy-3)    {};

% ==============================
% 2004 7
\node[concur,label={[align=center]below:Lock-free\\\cite{fomitchev2004lock}}]      (lockfree2)     at(\yx+7, \topy-2)    {};

% ==============================
% 2005 7.5
\node[default,label={[align=center]below:SkipQuadTree\\\cite{eppstein2005skip}}]      (quadtree)     at(\yx+7.5, \topy-2)    {};
\node[default,label={[align=center]below:BiasedSkipList\\\cite{bagchi2005biased}}]      (biased2)     at(\yx+7.5, \topy-3)    {};

% ==============================
% 2006 8
\node[concur,label={[align=center]below:ConcurrentSkipListMap\\Java\\}]      (java)     at(\yx+8, \topy-5)    {};
\node[concur,label={[align=center]below:Optimistic\\\cite{herlihy2006provably, herlihy2007simple}}]      (optim)     at(\yx+8, \topy-6)    {};
\node[other,label={[align=center]below:Video\\\cite{wang2006peer}}]      (video)     at(\yx+8, \topy-7)    {};


% ==============================
% 2007 8.5
\node[default,label={[align=center]below:Duality BST\\\cite{dean2007exploring}}]      (duality)     at(\yx+8.5, \topy-3)    {};
\node[other,label={[align=center]below:Skip-Graph\\\cite{aspnes2007skip}}]      (skipgraph)     at(\yx+8.5, \topy-1)    {};

% ==============================
% 2008 9
\node[other,label={[align=center]below:Tiara\\\cite{clouser2008tiara}}]      (tiara)     at(\yx+9, \topy-1)    {};

% ==============================
% 2009 9.5
\node[index,label={[align=center]below:Redis\\\cite{redis}}]      (redis)     at(\yx+9.5, \topy-5)    {};

% ==============================
% 2010 10
\node[index,label={[align=center]below:MemSQL\\\cite{memsql}}]      (memsql)     at(\yx+10, \topy-2)    {};

% ==============================
% 2011 10.5
\node[other,label={[align=center]below:Corona\\\cite{nor2013corona}}]      (corona)     at(\yx+10.5, \topy-8)    {};
\node[concur, minimum size=2mm, label={[align=center]below:LevelDB\\\cite{ghemawat2011leveldb}}] (leveldb) at(\yx+10.5, \topy-5) {
        \begin{tikzpicture}
            \node[deter, minimum size=1.8mm, inner sep=0pt] {};
        \end{tikzpicture}
    };

% ==============================
% 2017 
\node[st-txt,label={[align=center]below:TA-Tree\\\cite{8014478}}]      (ta)     at(\ya,2)    {};
\node[st-curr,label={[align=center]below:V-Tree\\\cite{7930011}}]              (v)     at(\ya,0)    {};

\node[deter,label={[align=center]below:Cache-sensitive\\\cite{}}]      (cache)     at(\yx+1, \topy-1)    {};


% ==============================
% 2018
\node[s-txt,label={[align=center]below:FAST\\~\cite{8509257}}]              (fast)    at(\yb,1)    {};


% ==============================
% 2019:command=(c)

% ==============================
% 2020:command=(d)

% ==============================
% 2021 

% ==============================
% 2022


% ==============================
% 2023


% ==============================
% 2024


% ================================================================================================
% draw edge 

% ==============================
% parents
\path[->]   (spy) edge              node        {} (fast)
            (cir) edge              node        {} (ta) 
            (veb) edge              node        {} (ta) 
            (r) edge              node        {} (hgr) 
            (r) edge              node        {} (wr) 
            (sgrid) edge              node        {} (bigrid) 
            ;




% \node[state]          (q_1) [above right=of q_0] {$q_1$};
% \node[state]          (q_2) [below right=of q_0] {$q_2$};
% \node[state,accepting](q_3) [below right=of q_1] {$q_3$};

% \path[->] (q_0) edge              node        {0} (q_1)
%                 edge              node [swap] {1} (q_2)
%           (q_1) edge              node        {1} (q_3)
%                 edge [loop above] node        {0} ()
%           (q_2) edge              node [swap] {0} (q_3)
%                 edge [loop below] node        {1} ();

% ================================================================================================
% draw general node labels at the below
\node[st-past,label=right:ST-past]        (l1)    at (0, -3)     {};
\node[st-curr,label=right:ST-present]     (l2)    at (2, -3)      {};
\node[st-fut,label=right:ST-future]       (l3)    at (4, -3)      {};
\node[s-txt,label=right:SText]            (l4)    at (6, -3)      {};
\node[spatial,label=right:Spatial]        (l5)    at (8, -3)      {};
\node[st-txt,label=right:ST-Text]        (l6)    at (10, -3)      {};
\node[unknown,label=right:Unknwown]        (l7)    at (12, -3)      {};


% Draw horizontal line at the bottom
\draw[thick] (\yx, 0) -- (\yh, 0);

% Draw year labels beneath the horizontal line
\node at (\yx, -0.3) {1990};
\node at (\ya, -0.3) {1992};
\node at (\yx+2, -0.3) {1994};
\node at (\yx+3, -0.3) {1996};
\node at (\yx+4, -0.3) {1998};
\node at (\yx+5, -0.3) {2000};
\node at (\yx+6, -0.3) {2002};
\node at (\yx+7, -0.3) {2004};
\node at (\yx+8, -0.3) {2006};
\node at (\yx+9, -0.3) {2008};
\node at (\yx+10, -0.3) {2010};
\node at (\yx+11, -0.3) {2012};
\node at (\yx+12, -0.3) {2014};
\node at (\yx+13, -0.3) {2016};
\node at (\yx+14, -0.3) {2018};
\node at (\yx+15, -0.3) {2020};
\node at (\yx+16, -0.3) {2022};

% \node[] at (0, -2) {Pre '17};  % remove draw to 
% \draw [dashed] (\yx,-1.5) -- (\yx, 10);
\end{tikzpicture}
% }



% Copied from: https://shantoroy.com/latex/Draw-literature-survey-tree-in-latex/


